RepoProbe: Benchmarking Architecture-Aware Repository Comprehension with Checklists

The integration of Large Language Models (LLMs) into software engineering has shifted the focus from function-level generation to repository-scale assistance. However, existing benchmarks largely rely on bug reports from GitHub Issues, which often allow models to bypass genuine understanding via pattern matching on error logs. This misalignment under-measures Edit Bias, which refers to premature generation, where models prematurely propose code modifications instead of understanding the existing repository architecture. Furthermore, current LLM-as-a-Judge scalar scoring suffers from high variance and low interpretability. This work introduces RepoProbe, a novel benchmark for evaluating repository-level code understanding through open-ended Q&A using GitHub Discussions, which focuses on open-ended architectural inquiries rather than defect reporting. To ensure rigorous evaluation, we propose a Checklist-Based Verification Protocol that decomposes answers into atomic, verifiable facts, thereby replacing subjective ratings with objective verification. Our evaluation of state-of-the-art (SOTA) LLMs reveals a persistent gap between high clarity and evidencegrounded technical correctness. It also quantitatively confirms the prevalence of edit bias, in which models prioritize code generation instead of architectural analysis. Finally, we demonstrate that our verification protocol significantly improves evaluation reliability compared to traditional evaluations with scalar scoring.

==> algorithms/alg_checklist_eval.tex <==
\begin{algorithm}[t]
\caption{Checklist-based Verification}
\label{alg:checklist_eval}
\begin{algorithmic}[1]
\Require 
  $q$: Question, 
  $a_{\text{ref}}$: Reference Answer, 
  $a_{\text{gen}}$: Model-Generated Response, 
  $\mathcal{C}$: Checklist $\{(p_i, w_i, r_i)\}_{i=1}^{n}$
\Ensure 
  $S_{\text{total}}$: Total Score, 
  $\mathbb{E}$: Set of Rationales

\State $S_{\text{total}} \gets 0$
\State $\mathbb{E} \gets \emptyset$

\Comment{Construct evaluation context}
\State $\text{Context} \gets (q, a_{\text{ref}}, a_{\text{gen}})$

\Comment{Holistic verification pass}
\State $(s_1, e_1), \dots, (s_n, e_n) \gets \Phi(\text{Context}, \mathcal{C})$

\For{$i \gets 1$ \textbf{to} $n$}
    \State \textbf{Verify} $s_i \in \text{ValidScores}(r_i)$ \Comment{Enforce rubric constraints}
    \State $S_{\text{total}} \gets S_{\text{total}} + s_i$
    \State $\mathbb{E}.\text{add}(e_i)$
\EndFor

\State \textbf{Return} $S_{\text{total}}, \mathbb{E}$
\end{algorithmic}
\end{algorithm}

==> figures/figure_shortcut.tex <==
\begin{tikzpicture}[
    node distance=1.5cm,
    basic/.style={draw, rectangle, rounded corners, align=center, minimum height=1cm, font=\small},
    input/.style={basic, fill=gray!10, text width=5cm, drop shadow},
    process/.style={basic, fill=blue!10, text width=4cm, drop shadow},
    code/.style={basic, fill=green!10, text width=2.5cm, font=\ttfamily\scriptsize},
    arrow/.style={->, >=stealth, thick},
    dashed_arrow/.style={->, >=stealth, thick, dashed, color=red!70},
    label_text/.style={font=\bfseries\small, align=center}
]
% Left Side: Issue
\node[label_text] (issue_title) at (0, 0) {\textsc{Paradigm A: GitHub Issue} \\ (Defect-Centric)};
\node[input, below=0.3cm of issue_title] (issue_input) {
    \textbf{Input: Bug Report} \\
    \textit{``Crash in config.py line 42...''} \\
    (Contains Stack Trace)
};
\node[code, below=2.5cm of issue_input] (target_file_1) {config.py};
\draw[dashed_arrow] (issue_input.south) -- node[right, align=left, font=\footnotesize, color=red] {\textbf{Debugging Shortcut} \\ (Pattern Match)} (target_file_1.north);

% Right Side: Discussion
\node[label_text, right=4cm of issue_title] (discuss_title) {\textsc{Paradigm B: RepoProbe} \\ (Discussion-Centric)};
\node[input, below=0.3cm of discuss_title] (discuss_input) {
    \textbf{Input: Inquiry} \\
    \textit{``How do I feature-flag this?''} \\
    (No file paths)
};
\node[process, below=0.8cm of discuss_input] (reasoning) {
    \textbf{Semantic Mapping} \\
    \textit{Intent} $\rightarrow$ \textit{Architecture}
};
\node[code, below=0.8cm of reasoning] (target_file_2) {config.py};
\draw[arrow] (discuss_input.south) -- (reasoning.north);
\draw[arrow] (reasoning.south) -- (target_file_2.north);
% Separator
\draw[dashed, thick, gray!50] ($(issue_title.east)!0.5!(discuss_title.west) + (0, 1)$) -- ($(issue_title.east)!0.5!(discuss_title.west) - (0, 5)$);
\end{tikzpicture}


==> tables/table_checklist_structure.tex <==
\begin{table*}[t]
  \centering
  \caption{Checklist structure with reference-answer-derived knowledge items (total: 10 points).}
  \label{tab:checklist_structure}
  \small
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{p{3.5cm}p{1.3cm}p{10cm}}
    \toprule
    \textbf{Key point} & \textbf{Weight} & \textbf{Rubric (discrete score levels fixed at dataset construction)} \\
    \midrule
    Knowledge item 1\newline\textit{(multi-tier rubric)} & $w_1$ & \textbf{Full score} ($w_1$ pts): Completely addresses the key aspect identified in the reference answer. \\[-0.2em]
     & & \textbf{Intermediate score(s)} ($s_1$ pts, $0 < s_1 < w_1$): Partially correct, but missing important details required by the reference answer. The specific intermediate levels (e.g., $2$ out of $4$) are fixed when constructing the checklist. \\[-0.2em]
     & & \textbf{Zero} (0 pts): Missing, incorrect, or contradicts the reference answer. \\
    \addlinespace
    Knowledge item 2\newline\textit{(binary rubric)} & $w_2$ & \textbf{Full score} ($w_2$ pts): Correctly states the factual claim present in the reference answer. \\[-0.2em]
     & & \textbf{Zero} (0 pts): Fails to state the fact or states it incorrectly. \\
    \addlinespace
    \multicolumn{3}{c}{\textit{Additional knowledge items as needed, where $k \in \{1, 2, 3, 4\}$; each rubric is tailored to the specific reference answer.}} \\
    \addlinespace
    Knowledge item $k$ & $w_k$ & \textit{Rubric derived from the technical or factual content of the reference answer, using either a multi-tier or a binary scheme.} \\
    \midrule
    Clarity \& Organization\newline\textit{(fixed across all questions)} & 1 & \textbf{1 pt:} The response has a clear structure, well-organized hierarchy, uses concise and easy-to-understand language, and contains no hallucinations or factual errors. \\[-0.2em]
     & & \textbf{0 pts:} The response has a disorganized structure, uses obscure language, or contains hallucinations or factual errors. \\
    \bottomrule
    \multicolumn{3}{p{14.8cm}}{\small\textbf{Constraints:} the content-specific knowledge item weights satisfy $\sum_{i=1}^{k} w_i = 9$, where $k \in \{1, 2, 3, 4\}$ and each $w_i \in \mathbb{Z}^+$. Partial score values ($s_i$) are proposed during checklist generation and then fixed in the released checklist. Binary rubrics (no partial credit) are used for single-fact verification.}
  \end{tabular}%
  }
\end{table*}


==> tables/table_results_rq1_language.tex <==
\begin{table*}[t]
\centering
\caption{Overall Performance of LLMs on RepoProbe across programming languages, reported as percentages.}
\label{tab:table_RQ1_language}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccccccccc}
\toprule
Category & Model & Python & TypeScript & Lua & Shell & Go & Rust & QML & C\# & Swift & C++ & Ruby & JavaScript & Java & C & PHP \\
\midrule
\multirow{13}{*}{Closed-weight models}
& GPT-5.2 & 63.8 & 67.8 & 66.1 & 62.0 & 62.4 & 60.4 & 48.8 & 57.6 & 54.6 & 66.2 & 55.2 & 67.0 & 69.5 & 65.8 & 46.2 \\
& GPT-5.4 & 60.9 & 66.5 & 65.6 & 56.9 & 65.2 & 58.5 & 43.0 & 57.9 & 53.7 & 58.3 & 57.8 & 56.5 & 66.2 & 51.7 & 50.8 \\
& Claude Opus 4.5 & 60.7 & 63.9 & 64.4 & 59.6 & 55.2 & 48.9 & 47.0 & 50.3 & 44.4 & 56.9 & 52.6 & 49.6 & 66.2 & 58.3 & 59.2 \\
& Claude Opus 4.6 & 63.3 & 68.7 & 65.2 & 64.4 & 61.0 & 56.7 & 48.1 & 52.4 & 56.8 & 60.7 & 55.6 & 57.0 & 69.5 & 65.0 & 48.5 \\
& Claude Sonnet 4.6 & 62.3 & 67.7 & 62.8 & 61.3 & 61.7 & 56.1 & 46.7 & 48.2 & 52.0 & 55.9 & 56.7 & 47.0 & 68.1 & 60.8 & 48.5 \\
& Grok 4.2 & 57.1 & 62.7 & 58.0 & 57.8 & 58.0 & 57.0 & 46.7 & 53.3 & 49.3 & 56.6 & 54.1 & 48.7 & 53.8 & 52.5 & 55.4 \\
& Gemini 3 Flash & 54.6 & 58.9 & 67.3 & 52.4 & 52.3 & 58.9 & 44.4 & 53.3 & 43.9 & 55.9 & 57.0 & 48.7 & 64.8 & 45.8 & 44.6 \\
& Gemini 3 Pro & 52.2 & 56.3 & 57.4 & 52.0 & 48.1 & 47.2 & 40.2 & 48.5 & 41.7 & 51.7 & 48.1 & 49.1 & 54.8 & 45.8 & 42.3 \\
& Gemini 3.1 Pro & 50.5 & 60.9 & 61.2 & 53.1 & 53.1 & 55.0 & 43.0 & 54.8 & 41.5 & 57.6 & 51.9 & 47.0 & 61.0 & 55.0 & 46.9 \\
& Qwen3-Max & 29.6 & 31.6 & 28.9 & 28.4 & 31.6 & 17.0 & 14.4 & 23.3 & 18.0 & 19.7 & 30.0 & 23.5 & 35.7 & 42.5 & 16.9 \\
& Qwen3.5-Plus & 54.0 & 56.7 & 52.6 & 50.7 & 51.7 & 44.3 & 36.3 & 45.8 & 35.4 & 37.2 & 41.5 & 43.0 & 60.5 & 45.8 & 49.2 \\
& Doubao-Seed-1.8 & 47.0 & 45.2 & 44.6 & 41.8 & 42.3 & 46.5 & 30.0 & 44.5 & 32.0 & 38.3 & 48.9 & 51.3 & 43.8 & 45.8 & 36.2 \\
& Doubao-Seed-2.0-Pro & 48.2 & 51.7 & 50.0 & 48.1 & 48.4 & 46.3 & 27.4 & 41.8 & 40.5 & 38.3 & 48.5 & 47.8 & 49.0 & 44.2 & 41.5 \\
\midrule
\multirow{7}{*}{Open-weight models}
& GLM-4.7 & 51.2 & 57.6 & 54.8 & 50.6 & 48.8 & 43.0 & 40.5 & 50.9 & 46.3 & 43.8 & 44.8 & 42.6 & 54.8 & 54.2 & 46.9 \\
& GLM-5 & 56.6 & 62.5 & 62.5 & 52.6 & 57.0 & 46.5 & 38.6 & 47.2 & 43.9 & 49.7 & 48.9 & 46.5 & 63.8 & 55.0 & 51.5 \\
& DeepSeek-V3.2 & 53.6 & 56.5 & 57.1 & 53.8 & 54.2 & 47.8 & 46.0 & 47.6 & 50.7 & 45.9 & 47.8 & 49.6 & 55.2 & 55.8 & 47.7 \\
& Kimi-K2 & 49.7 & 49.6 & 46.1 & 48.7 & 46.1 & 46.3 & 26.5 & 39.1 & 39.8 & 35.9 & 48.1 & 37.8 & 51.4 & 54.2 & 40.8 \\
& Kimi-K2.5 & 55.7 & 62.0 & 55.5 & 53.6 & 53.8 & 51.3 & 36.0 & 49.7 & 52.9 & 45.5 & 43.0 & 46.1 & 52.9 & 50.0 & 50.8 \\
& MiniMax-M2.1 & 46.3 & 52.1 & 46.4 & 45.9 & 43.6 & 38.5 & 34.9 & 40.6 & 36.6 & 42.4 & 42.6 & 38.3 & 47.1 & 44.2 & 43.1 \\
& MiniMax-M2.5 & 45.4 & 53.1 & 46.2 & 49.8 & 47.5 & 37.6 & 30.2 & 46.1 & 32.9 & 31.0 & 41.9 & 32.2 & 40.0 & 45.8 & 41.5 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/table_results_rq1_taxonomy.tex <==
\begin{table*}[ht]
    \centering
    \caption{Cross-category performance on RepoProbe. For each code-understanding category, we report Overall for Overall Performance and Perfect for Perfect Solve Rate, reported as percentages. For each metric, Best results are bolded and second-best are underlined.}
    \label{tab:table_RQ1_taxonomy}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llcccccc}\toprule
 &  & \multicolumn{2}{c}{Project Architecture}& \multicolumn{2}{c}{Business Logic}& \multicolumn{2}{c}{Implementation Details}\\\midrule
        Category & Model &
        Overall& Perfect&
        Overall& Perfect&
        Overall& Perfect\\
        \midrule
        \multirow{13}{*}{Closed-weight models}
        & GPT-5.2 & 66.6 & 25.6 & 63.2 & 19.4 & 61.7 & 27.0 \\
        & GPT-5.4 & 67.8 & 30.1 & 66.7 & 21.3 & 59.4 & 24.6 \\
        & Claude Opus 4.5 & 57.2 & 20.5 & 60.6 & 20.6 & 57.2 & 21.8 \\
        & Claude Opus 4.6 & 61.5 & 24.4 & 61.1 & 22.2 & 62.1 & 27.8 \\
        & Claude Sonnet 4.6 & 59.3 & 25.3 & 63.2 & 27.0 & 58.8 & 26.9 \\
        & Grok 4.2 & 62.0 & 26.5 & 56.5 & 19.0 & 54.9 & 22.7 \\
        & Gemini 3 Flash & 53.1 & 16.9 & 56.5 & 19.0 & 55.9 & 22.9 \\
        & Gemini 3 Pro & 50.6 & 18.1 & 54.1 & 11.1 & 51.9 & 19.5 \\
        & Gemini 3.1 Pro & 57.2 & 20.5 & 54.3 & 20.6 & 52.7 & 21.8 \\
        & Qwen3-Max & 30.1 & 4.8 & 26.5 & 4.8 & 26.6 & 5.1 \\
        & Qwen3.5-Plus & 53.6 & 18.1 & 52.9 & 15.9 & 49.0 & 17.0 \\
        & Doubao-Seed-1.8 & 48.8 & 15.7 & 42.7 & 12.7 & 42.1 & 12.2 \\
        & Doubao-Seed-2.0-Pro & 46.7 & 14.5 & 50.8 & 12.7 & 45.3 & 15.0 \\
        \midrule
        \multirow{7}{*}{Open-weight models}
        & GLM-4.7 & 53.7 & 20.5 & 49.2 & 15.9 & 49.9 & 17.8 \\
        & GLM-5 & 53.4 & 13.3 & 56.8 & 19.0 & 55.1 & 22.4 \\
        & DeepSeek-V3.2 & 55.1 & 16.9 & 50.5 & 14.3 & 53.5 & 18.7 \\
        & Kimi-K2 & 49.0 & 15.7 & 41.4 & 11.1 & 46.9 & 16.7 \\
        & Kimi-K2.5 & 53.9 & 24.1 & 54.6 & 12.7 & 54.3 & 21.0 \\
        & MiniMax-M2.1 & 49.0 & 13.3 & 40.3 & 9.5 & 43.0 & 12.7 \\
        & MiniMax-M2.5 & 47.8 & 19.3 & 43.3 & 7.9 & 43.4 & 14.7 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/table_results_rq1_theme.tex <==
\begin{table*}[t]
\centering
\caption{Overall performance across repository themes, reported as percentages. For each theme, best results are bolded and second-best are underlin}
\label{tab:table_RQ1_theme}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccc}
\toprule
Category & Model & LLM Framework & Cloud DevOps & Developer SDK & Editor UI & Monitoring Tools & Desktop Apps & Data Processing & Security \\
\midrule
\multirow{13}{*}{Closed-weight models}
& GPT-5.2 & 61.1 & 64.4 & 61.7 & 62.0 & 66.6 & 67.5 & 58.9 & 64.4 \\
& GPT-5.4 & 60.5 & 62.4 & 60.4 & 58.6 & 67.0 & 57.8 & 57.8 & 60.6 \\
& Claude Opus 4.5 & 58.4 & 60.5 & 55.7 & 60.1 & 58.0 & 51.2 & 52.6 & 61.1 \\
& Claude Opus 4.6 & 62.7 & 66.7 & 59.7 & 60.1 & 65.0 & 56.7 & 56.7 & 68.4 \\
& Claude Sonnet 4.6 & 61.4 & 65.9 & 58.7 & 58.0 & 65.2 & 52.7 & 51.1 & 64.1 \\
& Grok 4.2 & 57.0 & 60.2 & 53.5 & 55.3 & 61.6 & 53.3 & 54.1 & 63.0 \\
& Gemini 3 Flash & 54.7 & 57.2 & 55.6 & 56.8 & 55.9 & 46.5 & 54.3 & 57.6 \\
& Gemini 3 Pro & 49.9 & 53.1 & 51.6 & 52.5 & 52.7 & 48.5 & 46.1 & 52.4 \\
& Gemini 3.1 Pro & 50.6 & 57.5 & 55.8 & 54.0 & 57.0 & 46.3 & 53.7 & 58.7 \\
& Qwen3-Max & 27.2 & 34.4 & 25.1 & 24.4 & 31.4 & 22.9 & 27.6 & 28.4 \\
& Qwen3.5-Plus & 54.0 & 54.5 & 48.6 & 48.4 & 50.9 & 37.9 & 41.7 & 51.4 \\
& Doubao-Seed-1.8 & 45.2 & 43.0 & 41.2 & 41.5 & 46.8 & 46.0 & 44.3 & 45.2 \\
& Doubao-Seed-2.0-Pro & 46.6 & 53.2 & 44.7 & 44.0 & 50.2 & 45.8 & 44.6 & 47.9 \\
\midrule
\multirow{7}{*}{Open-weight models}
& GLM-4.7 & 49.2 & 50.9 & 49.2 & 51.3 & 53.4 & 46.5 & 47.4 & 60.5 \\
& GLM-5 & 54.3 & 59.3 & 52.2 & 53.2 & 61.4 & 49.2 & 48.5 & 63.0 \\
& DeepSeek-V3.2 & 51.0 & 54.8 & 52.5 & 53.8 & 56.8 & 52.3 & 46.7 & 56.0 \\
& Kimi-K2 & 47.2 & 48.4 & 43.0 & 43.0 & 51.4 & 42.3 & 44.3 & 51.6 \\
& Kimi-K2.5 & 54.0 & 58.3 & 53.9 & 49.7 & 59.3 & 46.5 & 44.6 & 63.5 \\
& MiniMax-M2.1 & 45.0 & 49.8 & 41.8 & 44.2 & 43.4 & 42.5 & 41.1 & 50.3 \\
& MiniMax-M2.5 & 45.4 & 52.5 & 41.1 & 43.0 & 48.6 & 34.2 & 35.2 & 51.7 \\
\bottomrule
\end{tabular}%
}
\end{table*}
